Task-Driven Manipulation with Reconfigurable Parallel Robots

ReachBot, a proposed robotic platform, employs extendable booms as limbs for mobility in challenging environments, such as martian caves. When attached to the environment, ReachBot acts as a parallel robot, with reconfiguration driven by the ability to detach and re-place the booms. This ability enables manipulation-focused scientific objectives: for instance, through operating tools, or handling and transporting samples. To achieve these capabilities, we develop a two-part solution, optimizing for robustness against task uncertainty and stochastic failure modes. First, we present a mixed-integer stance planner to determine the positioning of ReachBot's booms to maximize the task wrench space about the nominal point(s). Second, we present a convex tension planner to determine boom tensions for the desired task wrenches, accounting for the probabilistic nature of microspine grasping. We demonstrate improvements in key robustness metrics from the field of dexterous manipulation, and show a large increase in the volume of the manipulation workspace. Finally, we employ Monte-Carlo simulation to validate the robustness of these methods, demonstrating good performance across a range of randomized tasks and environments, and generalization to cable-driven morphologies. We make our code available at our project webpage, https://stanfordasl.github.io/reachbot_manipulation/

==> results_table.tex <==
% I probably won't actually use this table (see the figure instead), but backing it up here in case I need it later
\begin{table*}[]
    \caption{Manipulation task performance}
    \label{tab:task_results}
    \centering
    \begin{tabular}{@{\extracolsep{4pt}}lcccccc@{}}
        \toprule
                         & \multicolumn{3}{c}{Single-wrench task} & \multicolumn{3}{c}{Multi-wrench task}                                                                      \\
        \cmidrule{2-4}
        \cmidrule{5-7}
                         & Success                                & Fail - Geometric                      & Fail - Stochastic & Success & Fail - Geometric & Fail - Stochastic \\\midrule
        Naïve - Cables   & 16\%                                   & 81\%                                  & 3\%               & 0\%     & 98\%             & 2\%               \\
        Naïve - Booms    & 89\%                                   & 2\%                                   & 9\%               & 15\%    & 47\%             & 38\%              \\
        Optimal - Cables & 95\%                                   & 2\%                                   & 3\%               & 88\%    & 2\%              & 10\%              \\
        Optimal - Booms  & 100\%                                  & 0\%                                   & 0\%               & 90\%    & 0\%              & 10\%              \\ \bottomrule
    \end{tabular}
\end{table*}

